Surprising Efficacy of Fine-Tuned Transformers for Fact-Checking over Larger Language Models

In this paper, we explore the challenges associated with establishing an end-to-end fact-checking pipeline in a real-world context, covering over 90 languages. Our real-world experimental benchmarks demonstrate that fine-tuning Transformer models specifically for fact-checking tasks, such as claim detection and veracity prediction, provide superior performance over large language models (LLMs) like GPT-4, GPT-3.5-Turbo, and Mistral-7b. However, we illustrate that LLMs excel in generative tasks such as question decomposition for evidence retrieval. Through extensive evaluation, we show the efficacy of fine-tuned models for fact-checking in a multilingual setting and complex claims that include numerical quantities.

==> sigir2024-ai-editor-02.tex <==
\section{Related work}
\label{sec:related}

Automated fact-checking has become popular in research recently. However, there is relatively low adaption in the industry. There are existing tools such as browser plugin by~\citet{Botnevik:2020:SIGIRa} which can fact-check already written text. \citet{Wang:2023:arXiv} propose a tool for annotating the factual mistakes made by LLMs.  There are also tools for detecting hallucinations and factual mistakes made by LLMs, such as FactTool~\cite{Chern:2023:arXiva} and FAVA~\cite{Mishra:2024:arXiva}. While these are very sophisticated solutions, they do not focus on end-to-end fact-checking in a multilingual setting.


Majority of the fact-checking literature is focused on English language~\cite{Thorne:2018:arXiv,Guo:2022:JACL}. However, there are datasets for multilingual fact-checking \cite{Gupta:2021:ACL,Nielsen:2022:SIGIR}.
There is also recent survey on multilingual claim detection \citet{Panchendrarajan:2024:arXiv}. However, there is still a need for research regarding end-to-end fact-checking in multilingual setting.


